Statistical Arbitrage Risk Premium by Machine Learning

How to hedge factor risks without knowing the identities of the factors? We first prove a general theoretical result: even if the exact set of factors cannot be identified, any risky asset can use some portfolio of similar peer assets to hedge against its own factor exposures. A long position of a risky asset and a short position of a "replicate portfolio" of its peers represent that asset's factor residual risk. We coin the expected return of an asset's factor residual risk as its Statistical Arbitrage Risk Premium (SARP). The challenge in empirically estimating SARP is finding the peers for each asset and constructing the replicate portfolios. We use the elastic-net, a machine learning method, to project each stock's past returns onto that of every other stock. The resulting high-dimensional but sparse projection vector serves as investment weights in constructing the stocks' replicate portfolios. We say a stock has high (low) Statistical Arbitrage Risk (SAR) if it has low (high) R-squared with its peers. The key finding is that "unique" stocks have both a higher SARP and higher excess returns than "ubiquitous" stocks: in the cross-section, high SAR stocks have a monthly SARP (monthly excess returns) that is 1.101% (0.710%) greater than low SAR stocks. The average SAR across all stocks is countercyclical. Our results are robust to controlling for various known priced factors and characteristics.

==> elastic_net_discussions.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Discussions and details of the elastic-net estimator} 
\label{sec:ElasticNetDiscussion} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We introduce the optimization problem of the \textit{elastic-net} estimator developed by \cite{Zou2005}. Let $y$ be a $T \times 1$ vector, $\boldsymbol{X}$ be a $T \times N$ matrix and let $\beta$ be a $N \times 1$ vector. Consider the optimization problem, 
\begin{equation}
	\hat{\beta}_{\textrm{EN}} = \argmin_{\beta \in \R^N}\; \left\{ % 
		\frac{1}{2 T} \norm{ y - \boldsymbol{X}\beta }_2^2 + % 
	\lambda_1 \norm{\beta}_1 + % 
	\lambda_2 \norm{\beta}_2^2 %
	\right\}, 
	\quad
	\lambda_1, \lambda_2 \ge 0, 
	\label{eq:ElasticNet}
\end{equation}
where $\norm{x}_1 := \sum_{j=1}^N \abs{x_j}$ is the $L^1$-norm on $\R^N$, and $\norm{x}_2 := \sqrt{ \sum_{j=1}^N x_j^2 }$ is the $L^2$-norm on $\R^N$. In our application, $y$ will be a time series vector of $T$ days of returns of a particular stock, and $\boldsymbol{X}$ will be the concatenation of the time series of $N$ number of other stocks. Note this means there are $N + 1$ total number of stocks. 

The solution $\hat{\beta}_{\textrm{EN}}$ is called the \textit{elastic-net} estimator. This estimator encompasses the special cases of the \textit{ordinary least squares (OLS)} estimator (when $\lambda_1 = 0, \lambda_2 = 0$), \textit{least absolute shrinkage and selection operator (LASSO)} estimator of \cite{Tibshirani1996} (when $\lambda_1 > 0, \lambda_2 = 0$), and the \textit{ridge} estimator (when $\lambda_1 = 0, \lambda_2 > 0$). The hyperparameters $\lambda_1, \lambda_2$ control the strength of the $L^1$- and $L^2$-norm penalties, respectively. In this paper when we refer to the elastic-net estimator, we always refer to the case when $\lambda_1, \lambda_2$ are both strictly positive. In our actual implementation, we use a 3-fold \textit{cross-validation} procedure to empirically select the hyperparameters $\lambda_1, \lambda_2 > 0$.
\footnote{ 
To reduce the already lengthy computational time in estimating \eqref{eq:ElasticNet}, we cross-validate for only one hyperparameter rather than two by making the following simplifying assumption on $\lambda_1, \lambda_2$. We set $\lambda_1 = \lambda \ell$ and $\lambda_2 = \frac{1}{2} \lambda (1 - \ell)$, and set $\ell = 1/2$, and only cross-validate for the single $\lambda > 0$ parameter.  
}


In Theorem~\ref{thm:ThyReturnDecomp}, we motivated the need to \emph{linearly} regress a stock return $R_i$ onto the returns $\boldsymbol{R}_{-i}$ of all other stocks. The elastic-net estimator can actually be seen as a linear regression problem with constraints. By Lagrange-duality, \eqref{eq:ElasticNet} is identical to the following constrained least squares problem, 
\begin{equation}
\begin{aligned}
	& \min_{ \beta \in \R^N }   &     & \frac{1}{2T} \norm{ y - \boldsymbol{X} \beta }^2_2 \\ 
	& \textrm{subject to} 	    &     & \norm{\beta}_1 \le \eta_1, \\ 
	&                           &     & \norm{\beta}_2^2 \le \eta_2,  
\end{aligned}
\label{eq:ElasticNetConstrained} 
\end{equation}
for some $\eta_1, \eta_2 \ge 0$ that is dependent on the values of $\lambda_1, \lambda_2 \ge 0$. Most references in the statistical literature (e.g.\ \cite{Zou2005}) prefers the unconstrained Lagrangian-form \eqref{eq:ElasticNet} over the constrained optimization form \eqref{eq:ElasticNetConstrained} for theoretical and computational reasons. Here, we explicitly draw out the ``linear nature'' of the elastic-net estimator via \eqref{eq:ElasticNetConstrained} because Theorem~\ref{thm:ThyReturnDecomp} indeed predicts a linear relationship. 




==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );
   }
}

